A Logic for Choreographies

We explore logical reasoning for the global calculus, a coordination model based on the notion of choreography, with the aim to provide a methodology for specification and verification of structured communications. Starting with an extension of Hennessy-Milner logic, we present the global logic (GL), a modal logic describing possible interactions among participants in a choreography. We illustrate its use by giving examples of properties on service specifications. Finally, we show that, despite GL is undecidable, there is a significant decidable fragment which we provide with a sound and complete proof system for checking validity of formulae.

==> eptcsdata.tex <==
\providecommand{\firstpage}{29}
\providecommand{\publicationstatus}{K. Honda and A. Mycroft (Eds.): Programming Language\\
Approaches to Concurrency and communication-cEntric\\
Software 2010 (PLACES'10)\\
EPTCS 69, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.69.3}{10.4204/EPTCS.69.3}}
\pdfoutput=1

